Predicting Causes of Reformulation in Intelligent Assistants

Intelligent assistants (IAs) such as Siri and Cortana conversationally interact with users and execute a wide range of actions (e.g., searching the Web, setting alarms, and chatting). IAs can support these actions through the combination of various components such as automatic speech recognition, natural language understanding, and language generation. However, the complexity of these components hinders developers from determining which component causes an error. To remove this hindrance, we focus on reformulation, which is a useful signal of user dissatisfaction, and propose a method to predict the reformulation causes. We evaluate the method using the user logs of a commercial IA. The experimental results have demonstrated that features designed to detect the error of a specific component improve the performance of reformulation cause detection.

==> corpus.tex <==
\section{Corpus}
% \begin{table}[t]
%   % \begin{minipage}[t]{.5\textwidth}
%   \begin{center}
%     \begin{tabular}{lll}
%       \textbf{Task} & \textbf{\# of votes} & \textbf{\# of utterances} \\ \hline
%         Reformulation  & 5 & 2,068 \\
%           & 4 & 1,486 \\
%           & 3 & 1,218 \\
%           %      & 05  &  1562 \\
%           %      & 14  &  1114 \\
%           %      & 23  &   732 \\
%           % & 50  &   506 \\
%           % & 32  &   486 \\
%           % & 41  &   372 \\
%          & total  &  4,772 \\ \hdashline
%         Explicit  & 5 & 2,859 \\
%           & 4 & 1,190 \\
%           & 3 & 713 \\
%            % & 50  &  1542 \\
%            % & 05  &  1317 \\
%            % & 14 &   676 \\
%            % & 41  &   514 \\
%            % & 23  &   391 \\
%            % & 32  &    322 \\
%            & total  &  4,762 \\
%     \end{tabular}
%     \caption{The annotation results of crowdsourcing.}
%     \label{tab:crowdsourcing}
%   \end{center}
% % \end{minipage}
% \end{table}
We consisted two datasets of user logs of a commercial intelligent assistant\footnote{Because the intelligent assistant supports only Japanese, all utterances are made in Japanese. In this paper, we present English translations rather than the original Japanese to facilitate non-Japanese readers’ understanding.} for reformulation and positive/negative based on analysis shown in Section \ref{sec:analysis}. We randomly sampled 4,722 utterance pairs of ($U_1$, $U_2$) and corresponding information for reformulation dataset and 4,762 pairs for positive/negative dataset with the following five conditions.
First, $U_1$ and $U_2$ are text or voice inputs (\textit{i.e.} Quasi inputs such as autosuggest are excluded) .
Second, interval time between $U_1$ and $U_2$ is equal to or less than 30 minutes (followed previous research such as \citet{Jiang15} and \citet{Sano16}) .
In reformulation dataset, data where normalized Levenshtein edit distance \cite{Li07} between $U_1$ and $U_2$ equal to zero (\textit{i.e.} $U_1$ and $U_2$ are exactly same utterances) or more than 0.5 are excluded.
In positive/negative dataset, data where $U_2$ does not contain positive nor negative phrases in the categories listed in Table \ref{tab:posi_nega_type} are excluded.
Finally, data which lacks some information (\textit{e.g.} Voice data) or contains identical information is excluded.
As our focus is to predict user satisfaction from user utterances, we made efforts to exclude data where $U_2$ does not relate whether or not $U_1$ is SAT. First four conditions are filtering intended to make datasets high precision with reasonable recall. %また, 予測の際にはフィルタリングしなくても大丈夫なことを明記しておく.

Crowdsourcing workers are shown the triplets of texts of ($U_1$, $R$, $U_2$) and asked to annotate whether or not a user is satisfied with the system response $R$.
They are also instructed to estimate the intent of the user prior to the annotation. Note that voice inputs are converted into texts with automatic speech recognition.
To improve annotation quality, following two conditions are applied.
First, the labels are determined by the majority votes of five workers.
Second, workers who wrong the answer of the check problems are excluded.
The annotation results of reformulation dataset are 1,364 SAT data and 3,408 DSAT data, while those of positive/negative dataset are 2,378 SAT data and 2,384 DSAT data.
% The rates of data more than four out of five workers annotated same label are 74\% in reformulation dataset and 85\% in @ dataset. At first glance these rates seem not high, however, data where the annotation between workers are divided includes the confusing cases to determine user satisfaction. For example, one word utterance発話した本人でないと意図がわからないものや, 一語だけでそもそも意図がよくわからないものなども含まれており, 数値上ほど一致率が低いわけでない. 

